Identifying Causal Effects using Instrumental Time Series: Nuisance IV and Correcting for the Past

Instrumental variable (IV) regression relies on instruments to infer causal effects from observational data with unobserved confounding. We consider IV regression in time series models, such as vector auto-regressive (VAR) processes. Direct applications of i.i.d. techniques are generally inconsistent as they do not correctly adjust for dependencies in the past. In this paper, we outline the difficulties that arise due to time structure and propose methodology for constructing identifying equations that can be used for consistent parametric estimation of causal effects in time series data. One method uses extra nuisance covariates to obtain identifiability (an idea that can be of interest even in the i.i.d. case). We further propose a graph marginalization framework that allows us to apply nuisance IV and other IV methods in a principled way to time series. Our methods make use of a version of the global Markov property, which we prove holds for VAR(p) processes. For VAR(1) processes, we prove identifiability conditions that relate to Jordan forms and are different from the well-known rank conditions in the i.i.d. case (they do not require as many instruments as covariates, for example). We provide methods, prove their consistency, and show how the inferred causal effect can be used for distribution generalization. Simulation experiments corroborate our theoretical results. We provide ready-to-use Python code.

==> other_tex_files/commands.tex <==
% Capital letters
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\X}{{\mathbf X}} % Bold X
\renewcommand{\S}{{\mathbf S}} % Bold S
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\Gfull}{\mathcal{G}_{\text{full}}}

% Names
\DeclareMathOperator{\CIV}{CIV}
\DeclareMathOperator{\IV}{IV}
\DeclareMathOperator{\NIV}{NIV}
\newcommand{\iv}[2]{\IV_{#1\rightarrow #2}}
\newcommand{\civ}[2]{\CIV_{#1\rightarrow #2}}
\newcommand{\niv}[2]{\NIV_{#1\rightarrow #2}}


% Misc
\newcommand{\ind}[1]{\mathbbm{1}_{#1}} % Indicator function
\newcommand{\E}{\mathbb{E}}
\newcommand{\mat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\convP}{\stackrel{P}{\longrightarrow}}
\renewcommand{\vec}[1]{\left[ #1 \right]}
\newcommand{\vecin}[1]{[ #1 ]}
\newcommand{\cor}[1]{\langle #1 \rangle}
\newcommand{\indep}{\mbox{${}\perp\mkern-11mu\perp{}$}}
\newcommand{\notindep}{\centernot{\indep}\hspace{-2pt}}
\renewcommand{\epsilon}{\varepsilon}
\DeclareMathOperator*{\cov}{\operatorname{cov}}
\DeclareMathOperator*{\var}{\operatorname{var}}
\DeclareMathOperator*{\argmin}{{\arg\min}}
\DeclareMathOperator*{\rank}{\operatorname{rank}}
\DeclareMathOperator*{\diag}{{\operatorname{diag}}}
\DeclareMathOperator{\HAC}{HAC}
\DeclareMathOperator{\ID}{Id}



% Person commands
% \newcommand{\nikolaj}[1]{{\color{red}{\scriptsize N:}#1}}
% \newcommand{\seb}[1]{{\color{cyan} S: #1}}
% \newcommand{\rms}[1]{{\color{gray} remove (S): #1}}
% \newcommand{\rikke}[1]{{\color{orange} Rikke: #1}}
% \newcommand{\rmr}[1]{{\color{gray} Remove (R): #1}}
% \newcommand{\jonas}[1]{{\color{blue} #1}}
% \newcommand{\Jonas}[1]{{\color{blue} Jonas: #1}}
% \newcommand{\Rm}[1]{{\color{gray} Remove: #1}}
% \newcommand{\rmnik}[1]{{\color{gray} {\scriptsize N: #1}}}
% \newcommand{\new}[1]{{\color{olive!80!black}#1}}
% \newcommand{\rmj}[1]{{\color{gray} Remove (Jonas): #1}}
% \newcommand{\rmj}[1]{{\color{gray} Remove (Jonas): #1}}
% \newcommand{\old}[1]{{\color{gray} {\tiny #1}}}
% \newcommand{\old}[1]{{}}
% \newcommand{\new}[1]{#1}

% Define colors
\definecolor{MI_red}{HTML}{FC4F2C}
\definecolor{MXY_blue}{HTML}{135BB3}
\definecolor{highlight_green}{HTML}{429D6F}
\definecolor{highlight_yellow}{HTML}{E9B444}

% Graphs
\newcommand{\PA}{\operatorname{PA}}
\newcommand{\AN}{\operatorname{AN}}
\newcommand{\ND}[1]{\operatorname{ND}(#1)}
\newcommand{\DE}[1]{\operatorname{DE}(#1)}

% Renew subfigure
% \renewcommand{\thesubfigure}{Fig.~\arabic{figure}\alph{subfigure}}

\makeatletter
\newcommand{\mylabel}[2]{#2\def\@currentlabel{#2}\label{#1}}
\makeatother

==> other_tex_files/environments.tex <==
% \newtheorem{theorem}{Theorem}

%% Theorems
% \theoremstyle{plain}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}
% \newtheorem{example}{Example}
\crefname{assumption}{}{}%{Assumption}{Assumptions}
\Crefname{assumption}{}{}%{Assumption}{Assumptions}

\newtheorem*{assumption*}{Assumption} % Unnumbered assumptions

%% Unitalicized text
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}
 

% Cleveref should use oxford comma:
\newcommand{\creflastconjunction}{, and~}

%% Lists
\setlist[enumerate,1]{label={\roman*)}}

% Referencing assumptions
% Create new environment for assumption list, and set referencing as assumption instead of "Item"
% See this answer https://tex.stackexchange.com/questions/156049/how-can-i-get-cleveref-enumitem-to-print-not-item-e-but-proposition-1
\newlist{assumpenum}{enumerate}{1} % also creates a counter called 'assumpenumi'
\setlist[assumpenum]{label={(A\arabic*)},ref=(A\arabic*)}
\crefalias{assumpenumi}{assumption} 

% Referencing alternative assumptions
\newlist{alt-assumpenum}{enumerate}{1} % also creates a counter called 'alt-assumpenumi'
\setlist[alt-assumpenum]{label={(A\arabic*')},ref=(A\arabic*')}
\crefalias{alt-assumpenumi}{assumption} 

% Alternative alternative assumptions (used for time heterogeneous effect)
\newlist{alt-alt-assumpenum}{enumerate}{1} % also creates a counter called 'alt-alt-assumpenumi'
\setlist[alt-alt-assumpenum]{label={(A\arabic**)},ref=(A\arabic**)}
\crefalias{alt-alt-assumpenumi}{assumption} 



%Cref naming for requirements
\newtheorem{requirement}{Requirement}
\crefname{requirement}{requirement}{requirements}
\Crefname{requirement}{Requirement}{Requirements}

% Requirements for CIV 
\newlist{civenum}{enumerate}{1} % also creates a counter called 'assumpenumi'
% \setlist[civenum]{label={(CIV\arabic*)},ref=(CIV\arabic*)}
\setlist[civenum]{label={(CIV\arabic*)},ref=(CIV\arabic*),leftmargin=\widthof{(CIV3)}+\labelsep}
\crefalias{civenumi}{requirement} 

\newlist{alt-civenum}{enumerate}{1} % also creates a counter called 'assumpenumi'
\setlist[alt-civenum]{label={(CIV\arabic*')},ref=(CIV\arabic*'),leftmargin=\widthof{(CIV3)}+\labelsep}
\crefalias{alt-civenumi}{requirement} 

% Get "Assumptions (A1) -- (A4)" instead of "Assumptions (A1) to (A4)"
\crefrangelabelformat{assumption}{#3#1#4--#5#2#6}


==> other_tex_files/packages.tex <==
% Correct encoding
\usepackage[utf8]{inputenc}

% Solve conflict over \proof with amsthm and JRSS-B stylefile
% \let\proof\relax
% \let\endproof\relax

%AMS packages
\usepackage{amsmath, amsfonts, amssymb, amsthm}

%mathtools to get :=
\usepackage{mathtools}

%Graphics
\usepackage{graphicx}

%Hyperref
%https://en.wikibooks.org/wiki/LaTeX/Hyperlinks
% \usepackage{hyperref}

% Enable subfigures
\usepackage{subcaption}

%Package to get indicator function
\usepackage{bbm}

% Nice tables
\usepackage{booktabs}

% .. and to get bold calligraphic fonts
\usepackage{bm}

%\usepackage{fullpage}

%Coloured text, used for comments
\usepackage{xcolor}

%Enumerated lists with lowercase (i)
\usepackage{enumerate}
\usepackage[inline]{enumitem}
\newcounter{assumpCounter} % Counter for assumptions

% Graphs
\usepackage{tikz}
\usetikzlibrary{arrows}% To get more arrow heads
\usetikzlibrary{arrows.meta}
\usepackage{ifthen} % Get if-statements in figures

% References
\usepackage{natbib}

% Allow for algorithms
\usepackage{algorithm, algpseudocode, algorithmicx}

% Make strikethrough text
\usepackage[normalem]{ulem}
\newcommand{\st}[1]{\sout{#1}}

% Get not-independent correct
\usepackage{centernot}

% Restate theorems
\usepackage{thmtools}
\usepackage{thm-restate}
